Separating Retention from Extraction in the Evaluation of End-to-end Relation Extraction

State-of-the-art NLP models can adopt shallow heuristics that limit their generalization capability (McCoy et al., 2019). Such heuristics include lexical overlap with the training set in Named-Entity Recognition (Taill\'e et al., 2020) and Event or Type heuristics in Relation Extraction (Rosenman et al., 2020). In the more realistic end-to-end RE setting, we can expect yet another heuristic: the mere retention of training relation triples. In this paper, we propose several experiments confirming that retention of known facts is a key factor of performance on standard benchmarks. Furthermore, one experiment suggests that a pipeline model able to use intermediate type representations is less prone to over-rely on retention.

==> tables/ner_in_rel.tex <==
\begin{document}
    \begin{table}[!h]
    \centering
    \small
    
    \begin{tabularx}{\textwidth}{@{}l*{3}{Y}r*{3}{Y}r*{3}{Y}c@{}}
    
    \toprule
     & \multicolumn{3}{c}{NER in REL} &  & \multicolumn{3}{c}{NER Out REL} & & \multicolumn{3}{c}{ALL} \\
    \cline{2-4} \cline{6-8} \cline{10-12} 
    & Seen & Unseen & All & & Seen & Unseen & All &  & Seen & Unseen & All &  \\
    
    \midrule
    & \multicolumn{12}{c}{\textbf{ACE05}} \\
    \midrule
    
heuristic & 91.0$_{\stddev{\phantom{0.0}}}$ & - & 74.4$_{\stddev{\phantom{0.0}}}$ &  & 85.8$_{\stddev{\phantom{0.0}}}$ & - & 70.6$_{\stddev{\phantom{0.0}}}$ &  & 87.7$_{\stddev{\phantom{0.0}}}$ & - & 71.9$_{\stddev{\phantom{0.0}}}$ & \\


spert_entities & 93.8$_{\stddev{0.3}}$ & 67.8$_{\stddev{1.0}}$ & 89.1$_{\stddev{0.3}}$ &  & 87.8$_{\stddev{0.2}}$ & 70.9$_{\stddev{1.1}}$ & 84.8$_{\stddev{0.3}}$ &  & 89.9$_{\stddev{0.2}}$ & 69.8$_{\stddev{1.0}}$ & 86.3$_{\stddev{0.3}}$ & \\

    spert & 93.8$_{\stddev{0.3}}$ & 67.8$_{\stddev{0.9}}$ & 89.1$_{\stddev{0.4}}$ &  & 88.3$_{\stddev{0.4}}$ & 70.0$_{\stddev{1.4}}$ & 85.0$_{\stddev{0.3}}$ &  & 90.3$_{\stddev{0.3}}$ & 69.2$_{\stddev{0.9}}$ & 86.5$_{\stddev{0.3}}$ & \\

tabto_bert & 93.9$_{\stddev{0.3}}$ & 78.2$_{\stddev{1.7}}$ & 91.0$_{\stddev{0.5}}$ &  & 88.7$_{\stddev{0.5}}$ & 78.0$_{\stddev{1.5}}$ & 86.8$_{\stddev{0.6}}$ &  & 90.6$_{\stddev{0.4}}$ & 78.1$_{\stddev{1.5}}$ & 88.3$_{\stddev{0.6}}$ & \\

pure & 94.5$_{\stddev{0.3}}$ & 76.1$_{\stddev{0.8}}$ & 91.1$_{\stddev{0.3}}$ &  & 89.6$_{\stddev{0.2}}$ & 76.3$_{\stddev{0.6}}$ & 87.2$_{\stddev{0.2}}$ &  & 91.4$_{\stddev{0.1}}$ & 76.2$_{\stddev{0.6}}$ & 88.6$_{\stddev{0.1}}$ & \\

    \midrule
     & \multicolumn{12}{c}{\textbf{CoNLL04}} \\
    \midrule
    spert & 98.1$_{\stddev{0.5}}$ & 88.3$_{\stddev{0.4}}$ & 93.3$_{\stddev{0.3}}$ &  & 92.2$_{\stddev{1.1}}$ & 70.2$_{\stddev{0.5}}$ & 80.3$_{\stddev{0.4}}$ &  & 96.1$_{\stddev{0.6}}$ & 81.3$_{\stddev{0.3}}$ & 88.7$_{\stddev{0.3}}$ & \\

tabto_bert & 97.5$_{\stddev{0.5}}$ & 90.4$_{\stddev{0.8}}$ & 94.1$_{\stddev{0.6}}$ &  & 91.1$_{\stddev{2.5}}$ & 72.0$_{\stddev{0.6}}$ & 80.7$_{\stddev{1.2}}$ &  & 95.4$_{\stddev{0.7}}$ & 83.3$_{\stddev{0.3}}$ & 89.3$_{\stddev{0.4}}$ & \\

pure_cased & 97.7$_{\stddev{0.6}}$ & 89.0$_{\stddev{0.5}}$ & 93.5$_{\stddev{0.4}}$ &  & 91.8$_{\stddev{0.3}}$ & 69.2$_{\stddev{1.4}}$ & 79.5$_{\stddev{0.8}}$ &  & 95.8$_{\stddev{0.4}}$ & 81.4$_{\stddev{0.7}}$ & 88.5$_{\stddev{0.5}}$ & \\

spert_entities & 98.3$_{\stddev{0.3}}$ & 89.0$_{\stddev{1.0}}$ & 93.9$_{\stddev{0.6}}$ &  & 92.7$_{\stddev{1.0}}$ & 71.4$_{\stddev{1.7}}$ & 81.1$_{\stddev{1.1}}$ &  & 96.5$_{\stddev{0.4}}$ & 82.2$_{\stddev{1.1}}$ & 89.3$_{\stddev{0.7}}$ & \\

heuristic & 99.4$_{\stddev{\phantom{0.0}}}$ & - & 51.4$_{\stddev{\phantom{0.0}}}$ &  & 98.9$_{\stddev{\phantom{0.0}}}$ & - & 45.2$_{\stddev{\phantom{0.0}}}$ &  & 99.3$_{\stddev{\phantom{0.0}}}$ & - & 49.2$_{\stddev{\phantom{0.0}}}$ & \\
    
    \midrule
    & \multicolumn{12}{c}{\textbf{SciERC}} \\
    \midrule
 
    spert-scibert & 82.8$_{\stddev{1.0}}$ & 65.2$_{\stddev{0.4}}$ & 69.5$_{\stddev{0.3}}$ &  & 72.5$_{\stddev{2.0}}$ & 57.1$_{\stddev{1.2}}$ & 61.2$_{\stddev{1.0}}$ &  & 80.3$_{\stddev{0.7}}$ & 63.4$_{\stddev{0.3}}$ & 67.6$_{\stddev{0.2}}$ & \\
    
    pure & 82.0$_{\stddev{1.2}}$ & 64.0$_{\stddev{1.0}}$ & 68.1$_{\stddev{1.0}}$ &  & 68.2$_{\stddev{2.4}}$ & 57.2$_{\stddev{0.8}}$ & 59.9$_{\stddev{0.9}}$ &  & 78.7$_{\stddev{1.0}}$ & 62.5$_{\stddev{0.9}}$ & 66.2$_{\stddev{0.9}}$ & \\
 
    spert_entities_scibert & 83.6$_{\stddev{0.5}}$ & 64.3$_{\stddev{1.2}}$ & 68.7$_{\stddev{1.0}}$ &  & 68.6$_{\stddev{3.1}}$ & 56.2$_{\stddev{1.6}}$ & 59.3$_{\stddev{1.7}}$ &  & 80.0$_{\stddev{1.0}}$ & 62.5$_{\stddev{1.0}}$ & 66.6$_{\stddev{0.9}}$ & \\
    
    heuristic & 92.6$_{\stddev{\phantom{0.0}}}$ & - & 21.0$_{\stddev{\phantom{0.0}}}$ &  & 92.6$_{\stddev{\phantom{0.0}}}$ & - & 23.2$_{\stddev{\phantom{0.0}}}$ &  & 92.6$_{\stddev{\phantom{0.0}}}$ & - & 21.5$_{\stddev{\phantom{0.0}}}$ & \\

    \bottomrule
    
    \end{tabularx}
    \caption{NER RECALL in or Out of Relation}
    \label{table:ner_in_rel}
    \end{table}

\end{document}

==> tables/swap.tex <==
\begin{document}
    \begin{table}[!h]
    \centering
    \small
  
    \begin{tabularx}{\textwidth}{@{}ll*{2}{Y}r*{2}{Y}r*{2}{Y}c@{}}
    
    \toprule
    
     & & \multicolumn{2}{c}{NER} &  & \multicolumn{2}{c}{RE Boundaries} & & \multicolumn{2}{c}{RE Strict} \\
      
     \cline{3-4} \cline{6-7} \cline{9-10}
     & & Normal & Swap & & Normal & Swap & & Normal & Swap\\
     \midrule
     
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Kill}}} 
    
    & spert & 91.4$_{\stddev{1.2}}$ & 92.6$_{\stddev{1.2}}$ & 
            & 86.2$_{\stddev{1.4}}$ & 35.0$_{\stddev{5.6}}$ & 
            & 86.2$_{\stddev{1.4}}$ & 35.0$_{\stddev{5.6}}$  \\
            
    & spert_entities  & 91.6$_{\stddev{0.4}}$ & 91.7$_{\stddev{0.7}}$ &  
                    & 85.1$_{\stddev{0.9}}$ & 35.4$_{\stddev{6.5}}$ &
                    & 85.1$_{\stddev{0.9}}$ & 35.4$_{\stddev{6.5}}$ & \\
    
    & tabto_bert     & 92.0$_{\stddev{0.4}}$ & 92.8$_{\stddev{0.7}}$ &  
                    & 89.6$_{\stddev{1.3}}$ & 27.6$_{\stddev{3.8}}$ &  
                    & 89.6$_{\stddev{1.3}}$ & 27.6$_{\stddev{3.8}}$ &\\
                    
    & pure_cased    & 90.5$_{\stddev{0.6}}$ & 90.7$_{\stddev{0.5}}$ & 
                    & 84.1$_{\stddev{1.2}}$ & 52.3$_{\stddev{6.5}}$ & 
                    & 84.1$_{\stddev{1.2}}$ & 52.3$_{\stddev{6.5}}$ & \\
    
    \midrule
    
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Located}}} 
    & spert & 88.6$_{\stddev{1.1}}$ & 87.7$_{\stddev{1.1}}$ & 
            & 75.5$_{\stddev{1.4}}$ & 24.9$_{\stddev{9.2}}$ & 
            & 75.0$_{\stddev{2.0}}$ & 24.9$_{\stddev{9.2}}$\\
            
    & spert_entities  & 90.0$_{\stddev{0.7}}$ & 87.0$_{\stddev{2.1}}$ & 
                    & 78.3$_{\stddev{2.4}}$ & 30.3$_{\stddev{4.6}}$ &  
                    & 78.3$_{\stddev{2.4}}$ & 30.3$_{\stddev{4.6}}$ &    \\
    
    & tabto_bert    & 90.1$_{\stddev{1.5}}$ & 88.9$_{\stddev{0.8}}$ &
                    & 85.3$_{\stddev{3.9}}$ & 36.8$_{\stddev{6.3}}$ &  
                    & 85.3$_{\stddev{3.9}}$ & 36.1$_{\stddev{5.8}}$ &    \\
                    
    & pure_cased    & 89.0$_{\stddev{1.0}}$ & 83.7$_{\stddev{0.5}}$ &  
                    & 81.2$_{\stddev{2.6}}$ & 59.3$_{\stddev{3.0}}$ &  
                    & 81.2$_{\stddev{2.6}}$ & 59.3$_{\stddev{3.0}}$ &\\
        
    \bottomrule
    
    \end{tabularx}
    \caption{Swap}
    \label{table:swap}
    \end{table}

\end{document}

==> tables/swap_prf.tex <==
\begin{document}
    \begin{table}[!h]
    \centering
    \small
    
    \begin{tabularx}{\textwidth}{@{}lll*{3}{Y}r*{3}{Y}c@{}}
    
    \toprule
     
     & & & \multicolumn{3}{c}{NER} &  & \multicolumn{3}{c}{RE Strict} \\
      
     \cline{4-6} \cline{8-10}
     & & & P & R & F1 & & P & R & F1 \\
     \midrule
     
    \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Kill}}} 
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Normal}}} & spert & 91.7$_{\stddev{2.1}}$ & 91.0$_{\stddev{1.0}}$ & 91.4$_{\stddev{1.2}}$ &  & 88.1$_{\stddev{3.1}}$ & 84.4$_{\stddev{1.4}}$ & 86.2$_{\stddev{1.4}}$ & \\
    
    & & spert_entities & 91.7$_{\stddev{0.4}}$ & 91.5$_{\stddev{0.7}}$ & 91.6$_{\stddev{0.4}}$ &  & 82.9$_{\stddev{2.7}}$ & 87.6$_{\stddev{1.8}}$ & 85.1$_{\stddev{0.9}}$ & \\
    
    & & tabto_bert & 91.8$_{\stddev{0.6}}$ & 92.2$_{\stddev{0.5}}$ & 92.0$_{\stddev{0.4}}$ &  & 88.8$_{\stddev{1.6}}$ & 90.7$_{\stddev{3.3}}$ & 89.6$_{\stddev{1.3}}$ & \\
    
    & & pure_cased & 91.5$_{\stddev{0.9}}$ & 89.6$_{\stddev{0.6}}$ & 90.5$_{\stddev{0.6}}$ &  & 87.2$_{\stddev{2.1}}$ & 81.3$_{\stddev{1.1}}$ & 84.1$_{\stddev{1.2}}$ & \\
    
    \cline{2-10}
    %SWAP
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Swap}}} & spert & 92.6$_{\stddev{1.8}}$ & 92.6$_{\stddev{0.8}}$ & 92.6$_{\stddev{1.2}}$ &  & 33.0$_{\stddev{4.4}}$ & 37.3$_{\stddev{7.4}}$ & 35.0$_{\stddev{5.6}}$ & \\

    & & spert_entities & 91.3$_{\stddev{0.9}}$ & 92.1$_{\stddev{0.7}}$ & 91.7$_{\stddev{0.7}}$ &  & 31.8$_{\stddev{5.3}}$ & 40.0$_{\stddev{8.3}}$ & 35.4$_{\stddev{6.5}}$ & \\
    
    & & tabto_bert & 92.8$_{\stddev{0.8}}$ & 92.7$_{\stddev{0.9}}$ & 92.8$_{\stddev{0.7}}$ &  & 26.8$_{\stddev{3.6}}$ & 28.4$_{\stddev{4.1}}$ & 27.6$_{\stddev{3.8}}$ & \\
    
    & & pure_cased & 92.0$_{\stddev{0.5}}$ & 89.5$_{\stddev{1.0}}$ & 90.7$_{\stddev{0.5}}$ &  & 65.2$_{\stddev{6.0}}$ & 44.0$_{\stddev{7.4}}$ & 52.3$_{\stddev{6.5}}$ & \\
    
    
    
    
    \midrule
    
    \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Located in}}} 
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Normal}}} 
    &spert & 89.8$_{\stddev{1.2}}$ & 87.5$_{\stddev{1.5}}$ & 88.6$_{\stddev{1.1}}$ &  & 77.2$_{\stddev{2.8}}$ & 73.0$_{\stddev{3.0}}$ & 75.0$_{\stddev{2.0}}$ & \\

    & & spert_entities & 90.1$_{\stddev{0.8}}$ & 89.8$_{\stddev{1.5}}$ & 90.0$_{\stddev{0.7}}$ &  & 80.8$_{\stddev{3.7}}$ & 76.2$_{\stddev{3.2}}$ & 78.3$_{\stddev{2.4}}$ & \\
    
    & & tabto_bert & 90.1$_{\stddev{1.3}}$ & 90.0$_{\stddev{1.8}}$ & 90.1$_{\stddev{1.5}}$ &  & 93.0$_{\stddev{3.3}}$ & 78.9$_{\stddev{4.6}}$ & 85.3$_{\stddev{3.9}}$ & \\
    
    & & pure_cased & 88.6$_{\stddev{1.1}}$ & 89.4$_{\stddev{1.8}}$ & 89.0$_{\stddev{1.0}}$ &  & 89.3$_{\stddev{4.0}}$ & 74.6$_{\stddev{3.7}}$ & 81.2$_{\stddev{2.6}}$ & \\
    
    \cline{2-10}
    %SWAP
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Swap}}} 
    & spert & 87.3$_{\stddev{1.4}}$ & 88.0$_{\stddev{0.9}}$ & 87.7$_{\stddev{1.1}}$ &  & 34.8$_{\stddev{14.8}}$ & 19.5$_{\stddev{6.7}}$ & 24.9$_{\stddev{9.2}}$ & \\

    & & spert_entities & 86.7$_{\stddev{1.9}}$ & 87.4$_{\stddev{2.7}}$ & 87.0$_{\stddev{2.1}}$ &  & 38.0$_{\stddev{8.5}}$ & 25.4$_{\stddev{2.8}}$ & 30.3$_{\stddev{4.6}}$ & \\
    
    & & tabto_bert & 89.0$_{\stddev{0.6}}$ & 88.8$_{\stddev{0.9}}$ & 88.9$_{\stddev{0.8}}$ &  & 46.5$_{\stddev{6.6}}$ & 29.7$_{\stddev{5.7}}$ & 36.1$_{\stddev{5.8}}$ & \\
    
    & & pure_cased & 82.7$_{\stddev{0.8}}$ & 84.6$_{\stddev{0.8}}$ & 83.7$_{\stddev{0.5}}$ &  & 74.9$_{\stddev{7.6}}$ & 49.7$_{\stddev{4.7}}$ & 59.3$_{\stddev{3.0}}$ & \\
    
    \bottomrule
    
    \end{tabularx}
    \caption{Swap}
    \label{table:swap_prf}
    \end{table}

\end{document}
